Combining Observational and Randomized Data for Estimating Heterogeneous Treatment Effects

Estimating heterogeneous treatment effects is an important problem across many domains. In order to accurately estimate such treatment effects, one typically relies on data from observational studies or randomized experiments. Currently, most existing works rely exclusively on observational data, which is often confounded and, hence, yields biased estimates. While observational data is confounded, randomized data is unconfounded, but its sample size is usually too small to learn heterogeneous treatment effects. In this paper, we propose to estimate heterogeneous treatment effects by combining large amounts of observational data and small amounts of randomized data via representation learning. In particular, we introduce a two-step framework: first, we use observational data to learn a shared structure (in form of a representation); and then, we use randomized data to learn the data-specific structures. We analyze the finite sample properties of our framework and compare them to several natural baselines. As such, we derive conditions for when combining observational and randomized data is beneficial, and for when it is not. Based on this, we introduce a sample-efficient algorithm, called CorNet. We use extensive simulation studies to verify the theoretical properties of CorNet and multiple real-world datasets to demonstrate our method's superiority compared to existing methods.

==> authors.tex <==
\author{\name Tobias Hatt  \email thatt@ethz.ch  \\
       \addr ETH Zurich\\
       Weinbergstrasse, Zurich, Switzerland
       \AND
       \name Alicia Curth \email amc253@damtp.cam.ac.uk \\
       \addr University of Cambridge\\
       Wilberforce Rd, Cambridge, UK
        \AND
       \name Jeroen Berrevoets \email jeroen.berrevoets@damtp.cam.ac.uk \\
       \addr University of Cambridge\\
      Wilberforce Rd, Cambridge, UK
      \AND
       \name Stefan Feuerriegel \email sfeuerriegel@ethz.ch \\
       \addr ETH Zurich\\
       Weinbergstrasse, Zurich, Switzerland
        \AND
       \name Mihaela van der Schaar \email mv472@damtp.cam.ac.uk \\
       \addr University of Cambridge\\
       Wilberforce Rd, Cambridge, UK
}

==> jmlr_coverletter.tex <==
% !TEX program = pdflatex
\input{jmlr_coverletter_preamble.tex}

\begin{document}
\hfill{\today}

Journal of Machine Learning Research

\bigskip

Dear Editors:

We are writing to submit our manuscript ``\red{Combining Observational and Randomized Data for Estimating Heterogeneous Treatment Effects}'' to the \emph{Journal of Machine Learning Research}.

Our manuscript studies \red{how to estimate heterogeneous treatment effects by combining data from randomized controlled trials and data from observational studies}, which is important because \red{relying on either of the two kinds of data requires strong assumptions such as ``no unmeasured confounders''}.

This paper has not been published at any other venues.

We suggest the following action editors and referees for our submission.

Action Editors:
\begin{itemize}
    \item \red{David Sontag, MIT (dsontag@mit.edu)}
    \item \red{Victor Chernozhukov, MIT (vchern@mit.edu)}
    \item \red{Joris Mooij, University of Amsterdam (j.m.mooij@uva.nl)}
    \item \red{Peter Spirtes, Carnegie Mellon University (ps7z@andrew.cmu.edu)}
    \item \red{David Jensen, University of Massachusetts Amherst (jensen@cs.umass.edu)}
    \item \red{Vanessa Didelez, University of Bremen (didelez@leibniz-bips.de)}
    \item \red{Silvia Chiappa, DeepMind (chiappa.silvia@gmail.com)}
    \item \red{Edoardo Airoldi, Harvard University (airoldi@fas.harvard.edu)}
    \item \red{Silvia Chiappa, DeepMind (chiappa.silvia@gmail.com)}
\end{itemize}

Reviewers:
\begin{itemize}
    \item \red{Fredrik Johansson, Chalmers University of Technology (fredrik.johansson@chalmers.se)}
    \item \red{Victor Veitch, University of Chicago (vveitch@statistics.uchicago.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
    \item \red{First Lastname, Institution (first.lastname@institution.edu)}
\end{itemize}

Our submission has the following keywords: \red{Heterogeneous treatment effects}, \red{randomized controlled trials}, \red{observational data}, \red{neural networks}, \red{representation learning}.

As the corresponding author, I confirm that none of the co-authors listed below have a conflict of interest with the action editors and referees I suggest above. Further, I confirm that all co-authors below consent to my submission of this manuscript to the \emph{Journal of Machine Learning Research}.

\bigskip

Sincerely,

\medskip

\red{Tobias Hatt (ETH Zurich)}\\
%Order???\red{Alicia Curth (University of Cambridge)}\red{Jeroen Berrevoets (University of Cambridge)}\\
\red{Stefan Feuerriegel (ETH Zurich \&  Ludwig Maximilian University of Munich)}\\
\red{Mihaela van der Schaar (University of Cambridge \& UCLA \& Alan Turing Institute)}

\end{document}







































